Coarse Wage-Setting and Behavioral Firms

This paper shows that the bunching of wages at round numbers is partly driven by firm coarse wage-setting. Using data from over 200 million new hires in Brazil, I first establish that contracted salaries tend to cluster at round numbers. Then, I show that firms that tend to hire workers at round-numbered salaries have worse market outcomes. Next, I develop a wage-posting model in which optimization costs lead to the adoption of coarse rounded wages and provide evidence supporting two model predictions using two research designs. Finally, I examine some consequences of coarse wage-setting for relevant economic outcomes.

==> results/char_n.tex <==
\(N\)&&49,592&&242,985&&276,275&&1,841&&68,054&&69,852&\\


==> results/heurist_shr100_allf.tex <==
Share hired at mult 100&&0.388&\sym{***}&0.426&\sym{***}&0.240&\sym{***}&0.187&\sym{***}&0.393&\sym{***}&0.454&\sym{***}\\
&&(0.004&)&(0.004&)&(0.004&)&(0.003&)&(0.004&)&(0.004&)\\
Mean Dep. Var.&&0.354&&0.123&&0.344&&0.110&&0.421&&0.214&\\
N&&4,953,782&&3,646,479&&4,953,782&&3,646,479&&4,953,782&&3,646,479&\\


==> results/heurist_shr10_allf.tex <==
Share hired at a round number&&0.369&\sym{***}&0.438&\sym{***}&0.142&\sym{***}&0.099&\sym{***}&0.368&\sym{***}&0.448&\sym{***}\\
&&(0.003&)&(0.003&)&(0.003&)&(0.002&)&(0.003&)&(0.003&)\\
Mean Dep. Var.&&0.354&&0.123&&0.344&&0.110&&0.421&&0.214&\\
N&&4,953,782&&3,646,479&&4,953,782&&3,646,479&&4,953,782&&3,646,479&\\


==> results/ineq_bunch100_allf.tex <==
Bunching firm&&$-$0.017&\sym{***}&$-$0.142&\sym{***}&$-$0.085&\sym{***}&$-$0.029&\sym{***}\\
&&(0.001&)&(0.010&)&(0.006&)&(0.004&)\\
Mean Dep. Var.&&0.109&&1.739&&1.380&&1.236&\\
N&&1,622,410&&1,622,410&&1,622,410&&1,622,410&\\


==> results/ineq_bunch50_allf.tex <==
Bunching firm&&0.012&\sym{***}&0.115&\sym{***}&0.046&\sym{***}&0.038&\sym{***}\\
&&(0.000&)&(0.004&)&(0.002&)&(0.001&)\\
Mean Dep. Var.&&0.109&&1.739&&1.380&&1.236&\\
N&&1,622,410&&1,622,410&&1,622,410&&1,622,410&\\


==> results/ineq_bunch66_allf.tex <==
Bunching firm&&0.007&\sym{***}&0.077&\sym{***}&0.028&\sym{***}&0.029&\sym{***}\\
&&(0.000&)&(0.005&)&(0.003&)&(0.001&)\\
Mean Dep. Var.&&0.109&&1.739&&1.380&&1.236&\\
N&&1,622,410&&1,622,410&&1,622,410&&1,622,410&\\


==> results/ineq_bunch_allf_full.tex <==
Bunching firm&&$-$0.016&\sym{***}&$-$0.112&\sym{***}&$-$0.069&\sym{***}&$-$0.025&\sym{***}\\
&&(0.001&)&(0.013&)&(0.008&)&(0.004&)\\
Mean Dep. Var.&&0.174&&2.183&&1.602&&1.328&\\
N&&31,375,013&&31,375,013&&31,375,013&&31,375,013&\\


==> results/ineq_bunchyr_allf.tex <==
Bunching firm&&$-$0.010&\sym{***}&$-$0.076&\sym{***}&$-$0.043&\sym{***}&$-$0.021&\sym{***}\\
&&(0.001&)&(0.005&)&(0.003&)&(0.002&)\\
Mean Dep. Var.&&0.109&&1.739&&1.380&&1.236&\\
N&&1,622,410&&1,622,410&&1,622,410&&1,622,410&\\


==> results/ineq_shr100_allf.tex <==
Share hired at mult 100&&0.056&\sym{***}&0.503&\sym{***}&0.221&\sym{***}&0.156&\sym{***}\\
&&(0.001&)&(0.008&)&(0.005&)&(0.003&)\\
Mean Dep. Var.&&0.109&&1.739&&1.380&&1.236&\\
N&&1,622,410&&1,622,410&&1,622,410&&1,622,410&\\


==> results/ineq_shr10_allf.tex <==
Share hired at a round number&&0.030&\sym{***}&0.264&\sym{***}&0.116&\sym{***}&0.085&\sym{***}\\
&&(0.001&)&(0.006&)&(0.003&)&(0.002&)\\
Mean Dep. Var.&&0.109&&1.739&&1.380&&1.236&\\
N&&1,622,410&&1,622,410&&1,622,410&&1,622,410&\\


==> results/perf_shr100_allf.tex <==
Share hired at mult 100&&0.037&\sym{***}&0.005&\sym{***}&0.023&\sym{***}&$-$0.000&\\
&&(0.003&)&(0.002&)&(0.003&)&(0.001&)\\
Mean Dep. Var.&&0.353&&0.115&&0.016&&0.101&\\
N&&20,281,312&&20,281,312&&1,381,246&&1,752,411&\\


==> results/perf_shr10_allf.tex <==
Share hired at a round number&&0.010&\sym{***}&$-$0.004&\sym{***}&$-$0.002&&0.002&\sym{*}\\
&&(0.002&)&(0.001&)&(0.002&)&(0.001&)\\
Mean Dep. Var.&&0.353&&0.115&&0.016&&0.101&\\
N&&20,281,312&&20,281,312&&1,381,246&&1,752,411&\\


==> results/reg_mult1000_lcdf_hiring.tex <==
Firm hiring experience (logs)&&$-$0.642&\sym{***}&0.735&\sym{***}&$-$0.007&\sym{***}&$-$0.008&\sym{***}\\
&&(0.071&)&(0.062&)&(0.001&)&(0.001&)\\


==> results/reg_mult1000_lfirm_size.tex <==
Firm size (logs)&&$-$0.943&\sym{***}&$-$0.069&&$-$0.004&\sym{***}&0.002&\sym{***}\\
&&(0.034&)&(0.109&)&(0.000&)&(0.001&)\\


==> results/reg_mult1000_logcpi.tex <==
Consumer price index (logs)&&0.640&\sym{***}&0.511&\sym{***}&0.017&\sym{***}&0.021&\sym{***}\\
&&(0.016&)&(0.018&)&(0.000&)&(0.001&)\\


==> results/reg_mult1000_potential_exp.tex <==
Worker Potential experience&&0.513&\sym{***}&0.271&&0.037&\sym{***}&0.041&\sym{***}\\
&&(0.171&)&(0.189&)&(0.001&)&(0.001&)\\


==> results/reg_mult1000_schooling.tex <==
Worker Educational attainment&&0.761&\sym{**}&0.755&\sym{*}&0.045&\sym{***}&0.051&\sym{***}\\
&&(0.317&)&(0.321&)&(0.001&)&(0.001&)\\


==> results/reg_mult100_lcdf_hiring.tex <==
Firm hiring experience (logs)&&$-$0.876&\sym{***}&0.375&\sym{***}&$-$0.022&\sym{***}&$-$0.008&\sym{***}\\
&&(0.042&)&(0.116&)&(0.001&)&(0.001&)\\


==> results/reg_mult100_lfirm_size.tex <==
Firm size (logs)&&$-$0.973&\sym{***}&$-$0.757&\sym{***}&$-$0.004&\sym{***}&$-$0.009&\sym{***}\\
&&(0.021&)&(0.091&)&(0.000&)&(0.001&)\\


==> results/reg_mult100_logcpi.tex <==
Consumer price index (logs)&&0.329&\sym{***}&0.033&&0.042&\sym{***}&0.042&\sym{***}\\
&&(0.022&)&(0.023&)&(0.000&)&(0.001&)\\


==> results/reg_mult100_potential_exp.tex <==
Worker Potential experience&&0.418&\sym{**}&$-$0.411&\sym{**}&0.053&\sym{***}&0.053&\sym{***}\\
&&(0.189&)&(0.188&)&(0.000&)&(0.001&)\\


==> results/reg_mult100_schooling.tex <==
Worker Educational attainment&&0.825&\sym{**}&0.828&\sym{**}&0.065&\sym{***}&0.069&\sym{***}\\
&&(0.256&)&(0.253&)&(0.001&)&(0.001&)\\


==> results/reg_mult10_potential_exp.tex <==
Worker Potential experience&&$-$0.833&\sym{***}&$-$0.866&\sym{***}&0.034&\sym{***}&0.034&\sym{***}\\
&&(0.095&)&(0.071&)&(0.000&)&(0.001&)\\


==> results/reg_mult10_schooling.tex <==
Worker Educational attainment&&0.892&\sym{***}&0.917&\sym{***}&0.036&\sym{***}&0.037&\sym{***}\\
&&(0.199&)&(0.167&)&(0.000&)&(0.001&)\\


==> results/sticky_bunch100_allf.tex <==
Bunching firm&&0.187&\sym{***}\\
&&(0.006&)\\
Mean Dep. Var.&&0.263&\\
N&&4,953,782&\\


==> results/sticky_bunch50_allf.tex <==
Bunching firm&&0.039&\sym{***}\\
&&(0.001&)\\
Mean Dep. Var.&&0.263&\\
N&&4,953,782&\\


==> results/sticky_bunch66_allf.tex <==
Bunching firm&&0.057&\sym{***}\\
&&(0.002&)\\
Mean Dep. Var.&&0.263&\\
N&&4,953,782&\\


==> results/sticky_bunch_allf.tex <==
Bunching firm&&0.132&\sym{***}\\
&&(0.003&)\\
Mean Dep. Var.&&0.263&\\
N&&4,953,782&\\


==> results/sticky_bunch_bigf.tex <==
Bunching firm&&0.158&\sym{***}\\
&&(0.016&)\\
Mean Dep. Var.&&0.250&\\
N&&4,155,671&\\


==> results/sticky_bunchyr_allf.tex <==
Bunching firm&&0.099&\sym{***}\\
&&(0.003&)\\
Mean Dep. Var.&&0.263&\\
N&&4,953,782&\\


==> results/sticky_shr100_allf.tex <==
Share hired at mult 100&&0.135&\sym{***}\\
&&(0.004&)\\
Mean Dep. Var.&&0.263&\\
N&&4,953,782&\\


==> results/sticky_shr10_allf.tex <==
Share hired at a round number&&0.085&\sym{***}\\
&&(0.003&)\\
Mean Dep. Var.&&0.263&\\
N&&4,953,782&\\

